ACE: an Accurate and Cost-Effective Measurement System in SDN

Packet-level traffic measurement is essential in applications like QoS, traffic engineering, or anomaly detection. Software-Defined Networking (SDN) enables efficient and dynamic network configuration that we can deploy for fine-grained network state measurement. As the state changes dynamically, the sampling frequency must cope with that for accurate measurement. At the same time, we must consider the measurement cost, e.g., nodes' resource utilization. Existing works fall short in offering an optimal model to balance both the measurement accuracy and cost. We fill that gap by proposing ACE, an accurate and cost-effective measurement system that builds on a multi-objective optimization problem. As the optimization problem is NP-hard, we develop a heuristic. We solve the model using CPLEX; then implement a prototype of ACE in Mininet over real-world network topologies. The results confirm that ACE outperforms its counterparts in balancing both accuracy and cost.

==> background.tex <==
\section{Background} \label{background}


==> expSetup.tex <==
\section{ACE Design and Evaluation} \label{setup}

In this section, we first outline the architecture of ACE. Then, we present the evaluation setup and discussion on model evaluation and simulation results.

\textbf{ACE architecture:} 
The proposed greedy heuristic of ACE is deployed as an controller application at the Ryu. It manages a set of programmable switches (OVS) from the data plane. We deploy hybrid measurement scheme sFlow \cite{sflow} that consists of a sFlow-collector (resides at the control plane) and a set of sFlow-agents to offer both the active and passive measurements. The collector gathers the measurement, where sFlow agents installed at the switches samples counters with a rate configured by the ACE heuristic, APS. We consider sFlow instead of OpenFlow statistics as it depends on \textit{flow\_removed} messages, which impacts the accuracy as we observe in Figure~\ref{sflow_openflow}. In this evaluation, we use iperf \cite{iperf} to generate traffic for five source-destination pairs, each with an initial rate of one Mbps and double it at every ten seconds. Thus, the total network utilization is five Mbps initially. We also set the flow entry's hard timeout to five and fifteen seconds.

\begin{figure}[!t]
    \centerline{\includegraphics[width=0.95\textwidth]{figure/accuracy_of.png}}
    \caption{The measurement granularity of OpenFlow and sFlow \cite{remon}. }
    \label{sflow_openflow}
\end{figure}



\textbf{Evaluation setup:}

\textbf{Discussion on results:}

To test the performance of multiple link failure recovery and node failure recovery, we keep using ten testing pairs. But this time, we choose a testing node from yellow nodes. The reason of choosing these testing nodes is because they have more number of neighbours in each topology. We keep failing links one by one for each testing node separately until fail this node. We record recovery time, memory usage in terms of number of flow entries and operation cost in terms of number of adding and removing flow entries. To make network reachability, we increase FFG rules equals to number of neighbours instead of just two. So that we can recover from multiple link failure by just using Crankback. But for our ReMon, we still use two FFG entries.

To test the performance of adjusting polling frequency/sampling rate, we use real traffic data received by sFlow. We use \textit{iperf} to simulate high volume flows. We compare the performance of ReMon with sampling-on-demand and baseline approach in terms of the accuracy and resource consumption using CPLEX\cite{cplex}. The baseline approach is static polling frequency set as default. We also try different $a/b$ parameters to shows the best balance accuracy and cost
